autofz: Automated Fuzzer Composition at Runtime

Fuzzing has gained in popularity for software vulnerability detection by virtue of the tremendous effort to develop a diverse set of fuzzers. Thanks to various fuzzing techniques, most of the fuzzers have been able to demonstrate great performance on their selected targets. However, paradoxically, this diversity in fuzzers also made it difficult to select fuzzers that are best suitable for complex real-world programs, which we call selection burden. Communities attempted to address this problem by creating a set of standard benchmarks to compare and contrast the performance of fuzzers for a wide range of applications, but the result was always a suboptimal decision - the best-performing fuzzer on average does not guarantee the best outcome for the target of a user's interest. To overcome this problem, we propose an automated, yet non-intrusive meta-fuzzer, called autofz, to maximize the benefits of existing state-of-the-art fuzzers via dynamic composition. To an end user, this means that, instead of spending time on selecting which fuzzer to adopt, one can simply put all of the available fuzzers to autofz, and achieve the best, optimal result. The key idea is to monitor the runtime progress of the fuzzers, called trends (similar in concept to gradient descent), and make a fine-grained adjustment of resource allocation. This is a stark contrast to existing approaches - autofz deduces a suitable set of fuzzers of the active workload in a fine-grained manner at runtime. Our evaluation shows that autofz outperforms any best-performing individual fuzzers in 11 out of 12 available benchmarks and beats the best, collaborative fuzzing approaches in 19 out of 20 benchmarks. Moreover, on average, autofz found 152% more bugs than individual fuzzers, and 415% more bugs than collaborative fuzzing.

==> README <==
die: a paper template
=====================

## start

0. Prerequisites

  - Python 3.x
  - pygmentize

    $ pip install Pygments 

1. clone the git repo:

  - if you have none,

    $ git clone --depth=1 git@github.com:tsgates/die.git

  - if you have a git-repo to work on,

    $ git subtree add --squash git@github.com:tsgates/die.git master -P paper

  - or

    $ wget https://github.com/tsgates/die/releases/download/latest/die.tar.gz

2. build it:

    $ make
    p.pdf built @Tue May 20 20:38:19 EDT 2014
    
    (check p.pdf)

3. starting point, p.tex:

    $ grep -oP 'input{\K\w+' p.tex
    cmds
    rev
   *hdr
    abstract
   *ex
    intro
    overview
    design
    impl
    eval
    conclusion
    ack

  - hdr: includes title/author info
  - ex : includes latex examples

4. example latex

    $ git checkout example
    $ make

5. formatting rules (dependencies)

  - code/*.{c,cc,py,js ...} -> code/*.tex
  - fig/*.svg               -> fig/*.pdf
  - data/*.gp               -> fig/*.tex

  (see ex.tex for more details)

## tools

1. make a draft for revision

    $ make draft
    $ make watermark

2. abstract.txt (from abstract.tex)

    $ cat abstract.txt 

3. highlight changes, since the last submit

    $ make diff DIFF=HEAD@{}

4. spell check

    $ make spell

## Acknowledgment

This template contains a few files copied/stolen from the Internet and
mainly from my past collaborators (e.g., sty/*, conf.bib, some bin/),
which I couldn't keep track of their licenses.

==> background.tex <==
\section{Background}
\label{s:background}
\PP{AFL Bitmap}
AFL bitmap is a data structure that records the 
path explored by each round of fuzzing execution,
which measures code coverage.
One entry in the bitmap consists of an 8-bit counter and 
represents the number of times 
a certain path has been visited during execution.
In AFL, each bit of the counter is decoded into a specific range,
$1, 2, 3, \numrange[range-phrase = -]{4}{7},
\numrange[range-phrase = -]{8}{15}, 
\numrange[range-phrase = -]{16}{31},
\numrange[range-phrase = -]{32}{127}, 128^{+},$ respectively. 
For example, if the
MSB of the byte is set, 
the path has been visited more than 128 times.

\PP{Seed Synchronization}
Seed synchronization~\cite{clusterfuzz-google-web,afl} is initially proposed
to share interesting seeds generated by different instances of the same fuzzer.
Recently, it has been extended by ~\cite{chen19:enfuz}
to share unique test cases produced by different fuzzers. 
The purpose of this synchronization is to help 
a particular fuzzer consistently failing to make progress 
by introducing interesting inputs borrowed from other fuzzers.
Due to inherent randomness in fuzzing 
and the different mutation techniques of fuzzers,
the borrowed seed will allow each fuzzer to 
result in unique code coverage and vulnerability detection.




==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> eval-detail-cpu.tex <==

\setcounter{rowno}{0}

\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{fig/table5.pdf}}
\caption{\JH{Instead of showing details to one program, we can compare different target program with different resource allocation as a heat map. This will highlight how the autofuzz can distribute resource differently based on the target automatically. We can put this detail graph to the appendix}}
\label{f:XXX}
\end{figure}


==> eval-graph.tex <==



\begin{figure*}[htb]
  \begin{center}
    \begin{tabular}{ccc}
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/exiv2.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/ffmpeg.pdf} &
                                                                                             \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/imginfo.pdf} \\
      exiv2 & ffmpeg & imginfo \\
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/infotocap.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/mujs.pdf} &
                                                                                           \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/nm.pdf} \\
      infotocap & mujs & nm \\
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/pdftotext.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/tcpdump.pdf} &
                                                                                              \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/tiffsplit.pdf} \\
      pdftotext & tcpdump & tiffsplit
    \end{tabular}
  \end{center}
  \caption{Coverage Graph for \unifuzz}
  \label{f:eval-ratio-compare-unifuzz}
\end{figure*}

\begin{figure*}[htb]
  \begin{center}
    \begin{tabular}{ccc}
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/boringssl-2016-02-12.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/freetype2-2017.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/guetzli-2017-3-30.pdf} \\ 
      boringssl-2016-02-12 & freetype2-2017 & guetzli-2017-3-30  \\
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/json-2017-02-12.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/lcms-2017-03-21.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/libarchive-2017-01-04.pdf} \\ 
      json-2017-02-12 &  lcms-2017-03-21 & libarchive-2017-01-04 \\
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/libjpeg-turbo-07-2017.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/libpng.pdf} &
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/openssl-f.pdf} \\
      libjpeg-turbo-07-2017 & libpng & openssl-1.0.1f \\
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/openssl-d.pdf} & 
                                                                                                
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/re2-2014-12-09.pdf} &
                                                                                                     \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/sqlite-2016-11-14.pdf} \\
      openssl-1.0.2d &  re2-2014-12-09 sqlite-2016-11-14 \\
    \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/vorbis-2017-12-11.pdf} &
                                                                                                        \includegraphics[width=0.66\columnwidth]{data/ratio-300-24h-bitmap-density/woff2-2016-05-06.pdf} &
                                                                                                                                                                                                           \\
      vorbis-2017-12-11 & woff2-2016-05-06 \\
      \end{tabular}
  \end{center}
  \caption{Coverage Graph for \fts}
  \label{f:eval-fts-growth}
\end{figure*}

\begin{figure*}[htb]
  \begin{center}
    \includegraphics[width=2\columnwidth]{data/special/boringssl.pdf}
  \end{center}
  \caption{Rare case BoringSSL}
  \label{f:eval-rare-boringssl}
\end{figure*}

\begin{figure*}[htb]
  \begin{center}
    \includegraphics[width=2\columnwidth]{data/special/pdftotext.pdf}
  \end{center}
  \caption{Rare case pdftotext}
  \label{f:eval-rare-pdftotext}
\end{figure*}

==> latexmkrc <==
$bibtex = "bibtex -min-crossrefs=99";

push @cus_dep_list, "c tex 0 c2tex";
push @cus_dep_list, "cc tex 0 cc2tex";
push @cus_dep_list, "js tex 0 js2tex";
push @cus_dep_list, "py tex 0 py2tex";
push @cus_dep_list, "svg pdf 0 svg2pdf";
push @cus_dep_list, "plt tex 0 plt2tex";
push @cus_dep_list, "gp tex 0 gp2tex";
push @cus_dep_list, "dat gp 0 gp2tex";

sub c2tex { system("pygmentize -P tabsize=4 -P mathescape -f latex $_[0].c > $_[0].tex"); }
sub cc2tex { system("pygmentize -P tabsize=4 -P mathescape -f latex $_[0].cc > $_[0].tex"); }
sub js2tex { system("pygmentize -P linenos=1 -f latex $_[0].js > $_[0].tex"); }
sub py2tex { system("pygmentize -P tabsize=4 -P mathescape -f latex $_[0].py > $_[0].tex"); }
sub js2tex { system("pygmentize -P linenos=1 -f latex $_[0].js > $_[0].tex"); }
sub svg2pdf { system("inkscape --without-gui -f $_[0].svg -D -A $_[0].pdf"); }
sub gp2tex { system("gnuplot $_[0].gp"); }

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}



==> overview.tex <==
\section{Overview}
\label{s:overview}
\JH{NOTE:It should not really focus on EnFuzz \&c , but really highlight the design of \sys 
that allows automatic fuzzer selection. We don't want to focus on specific design 
of previous work.} 

In this section,
we explain the design of \sys  
that allows fine grained and non-intrusive fuzzer selection 
to achieve better performance.
Also, we explain several challenges 
need to be located in proposing \sys, a versatile meta-fuzzer,
and present our corresponding answers.

\PP{Why per workload not per program}
The key idea of \sys is dynamically deploying multiple set of fuzzers 
based on the workload at runtime, not per program.
Unlike other approaches
\sys can achieve better performance
with fine-grained selection at runtime.
In essence, 
it monitors the progress of individual fuzzers
and utilize them as a feedback
in its decision to select next set of fuzzers.
This versatility allows \sys to adapt different workload 
and adopt optimal fuzzers specialized in 
different workload. 
Although there is a overhead of context switching 
set of fuzzers based on workload, 
the performance gain achieved by deploying 
well-performing fuzzers outperforms the overhead. 
Furthermore, 
there is a trend in fuzzing execution
where one performing-well fuzzer 
will likely perform for a while
but not during entire execution.
If some fuzzers performs well, 
more resource will be allocated on them temporarily.
Therefore, it can accelerate well-performing fuzzers
and relegates the others.

\PP{Why meta-fuzzer considering runtime information}
Significant amount of researches
have been made to improve performance of one fuzzer.
However, still, there is no all-around fuzzer 
that can always achieve the best performance 
regardless of the fuzzing target. 
It indicates that each fuzzer is specialized in 
solving different problems in fuzzing. 
Recently, collaborative fuzzing introduces 
novel way to combine various fuzzers, but 
it does not utilize runtime information to reschedule 
the resource to the selected fuzzers. 
Above all else, 
it requires significant engineering effort to handpick fuzzers
well-suited to specific workload. 


\subsection{Challenges of \sys}
\label{ss:challenge}
\PP{When is an appropriate time to switch fuzzers}
\sys dynamically selects and switch to well-suited fuzzers 
by taking the runtime progress of fuzzers
as a feedback.
In other words,
\sys should be able to deal with workload changes
by adopting specific set of fuzzers 
among the baseline fuzzers.
To understand when is an appropriate time to switch fuzzers,
\sys should periodically measures 
the progress of the currently selected fuzzers. 
However, it incurs overhead to measure the progress.
If the switch operation happens at proper time 
the benefit of switching overcomes the overhead of runtime analysis.
However, if the switching happens too early,
it just incurs additional overhead of runtime analysis.
Also, when it happens too late, 
it cannot capture the trend 
and miss an opportunities to utilize other fuzzers
more suited to a changed workload. 

\PP{How to measure the fuzzing progress online.}
The main challenge is how can we collect and measure the 
progress of individual fuzzer at runtime. 
To fairly measure the progress of different fuzzers,
\sys requires unified criterion indicating progress of each fuzzer. 
\YF{1. AFL use afl bitmap coverage
    2. Angora use context-sensitive branch count
       (some info can be found in the angora paper section 2.1, 3.2)
    3. Libfuzzer use edge coverage}
However, 
depending on the technique and implementation of each fuzzer,
the underlying measurements can significantly vary. 
For example some fuzzers utilize edge coverage, 
but the others can use other information such as \XXX{PLEASE GIVE ME DETAIL}
to estimate current progress of fuzzers.
Moreover, the criteria should satisfy two requirements
to be adopted by \sys.
First, it should be concise and fast enough 
to report the progress changes in different fuzzers.
This is important because 
\sys utilizes the immediate trend changes 
to select next set of fuzzers. 
Second, it must be efficient not to incur severe overhead;
otherwise, it will waste valuable resource to measure progress
that could have been utilized by other fuzzer's executions.


\PP{Which fuzzers should the baseline include}
Another challenge is fruitless resource usages on substandard fuzzers
during runtime analysis. 
To automatically select subset of fuzzers
that performs well for particular workload, 
it requires data regarding all baseline fuzzers.
If \sys is too generous 
to allow excessive number of fuzzers 
to participate in the competition,
resource spent on analysis
can outweigh the advantage of considering various fuzzers
in the selection. 
However, if \sys is too restrictive 
to rule out beneficial candidates from the competition, 
it cannot achieve the best outcomes with 
well-suited fuzzers for particular workload. 
Therefore, the policy that determines 
which fuzzer should be included in the runtime analysis 
is paramount to achieve optimal outcome. 

\PP{How to efficiently distribute resource.}
In addition to automatic fuzzer selection capability,
dynamic resource adjustment among the selected fuzzer 
is one of the key contribution of \sys.
Unlike previous works that statically assign resources onetime
at initialization, 
\sys prioritizes specific fuzzer or set of fuzzers
by rescheduling the resources allocated to each fuzzer.
Therefore, the resource scheduling policy is dominant factor 
determining the efficiency of \sys.
For example, it can prioritize the best performant one 
or proportionally distribute resource based on 
progress of candidates.
We will provide the detail design and implementation of 
this decision policy in~\autoref{}.









